Data-driven Analysis of Gender Differences and Similarities in Scratch Programs

Block-based programming environments such as Scratch are an essential entry point to computer science. In order to create an effective learning environment that has the potential to address the gender imbalance in computer science, it is essential to better understand gender-specific differences in how children use such programming environments. In this paper, we explore gender differences and similarities in Scratch programs along two dimensions: In order to understand what motivates girls and boys to use Scratch, we apply a topic analysis using unsupervised machine learning for the first time on Scratch programs, using a dataset of 317 programs created by girls and boys in the range of 8-10 years. In order to understand how they program for these topics, we apply automated program analysis on the code implemented in these projects. We find that, in-line with common stereotypes, girls prefer topics that revolve around unicorns, celebrating, dancing and music, while boys tend to prefer gloomy topics with bats and ghouls, or competitive ones such as soccer or basketball. Girls prefer animations and stories, resulting in simpler control structures, while boys create games with more loops and conditional statements, resulting in more complex programs. Considering these differences can help to improve the learning outcomes and the resulting computing-related self-concepts, which are prerequisites for developing a longer-term interest in computer science.

==> content/relatedwork.tex <==
\section{Related Work}
\label{sec:rw}

Adams and Webster (2012) \cite{adams2012} conducted a study with 209 Alice and 113  \Scratch projects to examine the usage of basic concepts of programming such as variables, if-conditions, loops and dialog constructs in different project genres.  As a result, they found out that game projects contained more variables, if-statements, loop-statements than storytelling and music video projects. However, the presence of dialogue is in storytelling projects significantly higher than in games. The length of all three project types remain the same. Regarding gender differences, projects of girls contain more dialog messages than boys'. Highly interesting is that the stories of boys conatined significantyl more fire animatsions. The authors conclude that the kind of stroy elements boys and girls find interestings are differents, with boys facoring actions elements and girls dialog. %variables good in gaming because specific information about score etc. must be stroed. music videos have linear narrative structure where if statement is not needed. ; but conditional statements are essential for gameplay

Hsu (2014) \cite{hsu2014} examined gender differences in \Scratch game design from the \Scratch competition in 2013 with 46 participants. Her results showed that girls had better knowledge of counting loops, boys implemented more game specific code, in game projects, the girls implemented more positive feedback. Boys used also more built-in backgrounds and used slightly more motion-blocks. Girls used slightly more backgrounds and costumes than boys. Overall, boys implemented more game design mechanisms than girls.

In a case study of Sullivan and Umaschi Bers (2016) \cite{sullivan2016} boys performed significantly better in advanced robotic programming such as repeat-loops with KIWIE robotics kit than girls, but they performed equally well on other tasks such as basic programming concepts. 

Code smells and their impact on the understandability and simplicity of \Scratch programs are well studied \cite{hermans2016, hermans2016a}.  

In a previous study, Funke et al. (2017) \cite{funke2017a} investigated the gender differences in 127  \Scratch programs with the result that girls are more likely to use blocks of the looks-category while boys are using mostly blocks of the motion-category. Girls are more likely to program stories, which  require a particularly large number of looks blocks and have a lower level of comprehension, and boys are more likely to program games, which require a large number of motion blocks and have a higher level of comprehension. Overall, boys have almost twice as many different blocks as girls, which indicates that boys are more willing to experiment.

Aivaloglou and Hermans (2019)\cite{aivaloglou2019} conducted a study .. As a result, girls are more likely to use elements of storytelling and design. Contrary to the male students, female students preferred structured programming sessions, like to follow instructions, plan and think before implementing their idea. 

\cite{aivaloglou2019a} ...

Iskrenovic-Momcilovic (2019) \cite{iskrenovic-momcilovic2019} investigated the impact of pair programming in \Scratch.

Rubegni et al. (2020) \cite{rubegni2020} addressed the problem of stereotypical thinking with designing a Digital StoryTelling (DST) which should raise awareness. Therefore, workshops with 43 students to developed concepts for introducing a DST tool for raising awareness of gender role models and stereotypes. 

Using a web scraper, Moreno-Leon et al. (2020) \cite{moreno-leon2020} examined the different project types (genres) for their computational thinking score. Animations represent a lower level of difficulty than games. The authors conclude that it makes pedagogical sense to start computer science courses with the implementation of an animation and to increase the level of abstraction by implementing a game.

Rose et al (2020) \cite{p.rose2020} claimed that code smells -- especially duplicate code, large scripts and dead code -- can be reduced by using procedural abstraction. The authors propose a game design in \Scratch with the concrete example project "Pirate Plunder" and evaluated it using 91 children and the computational thinking score to learn this concept optimally and derive further learning goals from it. It is questionable to what extent the proposed project really motivates children to program under the aspect of gender.

The study by Papavlasopoulou et al. (2020)\cite{papavlasopoulou2020} used eye-tracking to investigate gender differences in programming activities among 8-17 year olds.  No statistically significant differences were found between girls and boys in terms of eye-tracking behaviour, learning growth and use of programming concepts. However, it was found that there were gender-specific strategies: Girls discussed more and collaborated more in the group, while boys started programming directly and focused more on it. Gender differences need to be taken into account in programming lessons, and thus also the importance of a positive self-concept of the girls must be taken into account.

 Amanullah and Bell (2019) \cite{amanullah2019} studied the progress of \Scratch users in their use of program concepts such as if or forever-statements. They noticed that more experienced users use variables, if, nestedif, repeat, and forever much more \Scratch than beginners. They conclude that users see \Scratch less as a programming language and use more simple features like costume changes. They see the reason for this in the teaching materials and the didactic approach.

Fields et al. (2017) \cite{fields2017} examined over 5,000 \Scratch users' use of programming concepts in relation to their level and time of activity, as well as by gender. Their results show that most \Scratch users use simple concepts such as loops and are female. In contrast, boys use more complex programming concepts such as boolean expressions.


Rubio et al. (2015) \cite{rubio2015a} found that girls and boys exhibit a different learning approach to programming as well as implement different pogramming concepts.


Richard and Kafai (2016) \cite{richard2016} investigated the diversity within the \Scratch community. They analysed data on project creators, content and comments. They found a high degree of diversity in age, geography and gender balance, but little diversity in cultural identity. 

Sullivan and Bers (2013) \cite{sullivan2013} introduced kindergarten children to the TangibleK Robtics Program and found only two significant differences: boys make the robotic material cleaner and program with if-statements. Since both genders performed equally well in the final project, the authors conclude that the boys have more exposure to conventional male toys and are therefore more interested in robotics and take more risks in programming than the girls.


